ShareDP: Finding k Disjoint Paths for Multiple Vertex Pairs

Finding k disjoint paths (kDP) is a fundamental problem in graph analysis. For vertices s and t, paths from s to t are said to be disjoint if any two of them share no common vertex except s and t. In practice, disjoint paths are widely applied in network routing and transportation. In these scenarios, multiple kDP queries are often issued simultaneously, necessitating efficient batch processing. This motivates the study of batch kDP query processing (batch-kDP). A straightforward approach to batch-kDP extends batch simple-path enumeration with disjointness checks. But this suffers from factorial computational complexity. An alternative approach leverages single-query algorithms that avoid this by replacing the graph with a converted version. However, handling each query independently misses opportunities for shared computation. To overcome these limitations, we propose ShareDP, an algorithm for batch-kDP that shares the computation and storage across kDPs. ShareDP merges converted graphs into a shared structure, then shares the traversals and operations from different queries within this structure. Extensive experiments on 12 real-world datasets confirm the superiority of ShareDP over comparative approaches.

==> tab/shareDP_condense.tex <==
\begin{algorithm}[t]
% \scriptsize
    \caption{ShareDP}
    \label{alg:shareDP}
    \KwIn{Set of $k$DP queries $Q$, original graph $G$, integer $k$}
    \KwOut{$k$ disjoint paths for each query $q \in Q$}
    
    Initialize \{$P$\}: Set $prehops$, $nexthops$, $isPinner$ to $\emptyset$, and initialize $isS$ and $isT$ according to the definition.\textit{\color{gray}// Initialize the merged split-graph. } \\
    \ForEach{$i$ $\in$ $1, \ldots, k$ \textit{\color{blue}/* Find the $i$th disjoint paths */}} 
    {
        \textit{\color{blue}/* Initialization for bidirectional BFS */} \\
        Initialize $s$-$seen$, $s$-$queue$, $s$-$nextqueue$ for forward BFS. Backward BFS uses analogous structures (e.g., $t$-$queue$). \\
        Initialize $joint$, $pred$, and $succ$ \textit{\color{gray}// $joint$: meeting points of forward and backward searches; $pred$/$succ$: path predecessors/successors.} \\
        $undone = Q$ \textit{\color{gray}// Queries that have not yet found the $i$th path.} \\
        
        \ForEach{$q \in Q$} 
        {
            $s$-$seen_{q.s} \cup= \{q\}$; $s$-$queue_{q.s} \cup= \{q\}$ \textit{\color{gray}// Mark $q.s$ as visited and enqueue it for forward search. Initialization for backward search is similar.} \\
        }

        \textit{\color{blue}/* Bidirectional BFS */} \\
        \While{$undone \neq \emptyset$ and $s$-$queue$ and $t$-$queue$ are not empty} 
        {
            \textit{\color{gray}/* Forward search */} \\
            \ForEach{\{$v$, $B$\} $\in s$-$queue$ \textit{\color{gray} // $B$ is a set of $k$DPs that need to expand $v$}}
            {
                $B = B \setminus undone$ \textit{\color{gray}// Skip queries that have already found the $i$th path.} \\
                \ForEach{\{$u$, $B'$\} $\in$ GetOutNeighbors($v$, $B$, $G$, \{$P$\}) \textit{\color{gray}// See Alg.~\ref{alg:get_nbr}.}} 
                {
                     $D = B' \setminus s$-$seen_u$ \textit{\color{gray}// Exclude queries that have already visited $u$.} \\
                     $s$-$seen_u \cup= D$; $pred_{u, v} \cup= D$ \textit{\color{gray}// Mark visited and record predecessor.} \\
                     $meet = D \cap t$-$seen_u$ \textit{\color{gray}// Found a path} \\
                     $joint_u \cup= meet$; $undone \setminus= meet$ \textit{\color{gray}// Mark queries as completed.} \\
                     $s$-$nextqueue_u \cup= (D \setminus meet)$ \textit{\color{gray}// Add to the queue.} \\
                }
            }
            Swap $s$-$queue$ and $s$-$nextqueue$ \\
            \textit{\color{gray}/* Backward search proceeds similarly to forward search. */}
        }

        \textit{\color{blue}/* Construct paths and update the merged split-graph */} \\
        Construct paths from $undone$, $joint$, $pred$, and $succ$. \\
        Update $prehops$, $nexthops$, and $isPinner$.\textit{\color{gray}// Adjust paths similar to flow augmentation in max-flow problem. } \\
    }
    
    Extract $k$ disjoint paths for each $q \in Q$ from path records and return the results. \\
    % \vspace{-2pt}
\end{algorithm}


